Hybridization of the Virtual Element Method for linear elasticity problems

We extend the hybridization procedure proposed in [Arnold, Brezzi, 1985, ESAIM: M2AN] to the Virtual Element Method for linear elasticity problems based on the Hellinger-Reissner principle. To illustrate such a technique, we focus on the 2D case, but other methods and 3D problems can be considered as well. We also show how to design a better approximation of the displacement field using a straightforward post-processing procedure. The numerical experiments confirm the theory for both two and three-dimensional problems.

==> conclusions.tex <==
\section{Conclusions}~\label{section:conclusion}
In the present work we have introduced the hybridization procedure of Virtual Element Methods for elasticity problems based on the Hellinger-Reissner functional. Following the guidelines of \cite{ArnoldBrezzi_1985}, we have also designed a suitable higher-order post-processed approximation for the displacement field.  
Event though the analysis has been presented for 2D problems, we developed a numerical test campaign to assess the behavior of this approach, including the 3D case, too.
Our numerical tests show that, within the framework of the VEM dicretization of the Hellinger-Reissner functional, the hybridization procedure is indeed a very effective way to solve the linear elastic problems, especially for 3D case.
